Computational Complexity of Certifying Restricted Isometry Property

Given a matrix $A$ with $n$ rows, a number $k<n$, and $0<\delta < 1$, $A$ is $(k,\delta)$-RIP (Restricted Isometry Property) if, for any vector $x \in \mathbb{R}^n$, with at most $k$ non-zero co-ordinates, $$(1-\delta) \|x\|_2 \leq \|A x\|_2 \leq (1+\delta)\|x\|_2$$ In many applications, such as compressed sensing and sparse recovery, it is desirable to construct RIP matrices with a large $k$ and a small $\delta$. Given the efficacy of random constructions in generating useful RIP matrices, the problem of certifying the RIP parameters of a matrix has become important. In this paper, we prove that it is hard to approximate the RIP parameters of a matrix assuming the Small-Set-Expansion-Hypothesis. Specifically, we prove that for any arbitrarily large constant $C>0$ and any arbitrarily small constant $0<\delta<1$, there exists some $k$ such that given a matrix $M$, it is SSE-Hard to distinguish the following two cases: - (Highly RIP) $M$ is $(k,\delta)$-RIP. - (Far away from RIP) $M$ is not $(k/C, 1-\delta)$-RIP. Most of the previous results on the topic of hardness of RIP certification only hold for certification when $\delta=o(1)$. In practice, it is of interest to understand the complexity of certifying a matrix with $\delta$ being close to $\sqrt{2}-1$, as it suffices for many real applications to have matrices with $\delta = \sqrt{2}-1$. Our hardness result holds for any constant $\delta$. Specifically, our result proves that even if $\delta$ is indeed very small, i.e. the matrix is in fact \emph{strongly RIP}, certifying that the matrix exhibits \emph{weak RIP} itself is SSE-Hard. In order to prove the hardness result, we prove a variant of the Cheeger's Inequality for sparse vectors.

==> reduction.tex <==

% !TEX root = main.tex


%\section{Hardness Results}
%
%Given any $d$-regular graph $G$, with adjacency matrix $A$, the Laplacian of $G$ is defined as $L = I - \frac{A}{d}$. From the basic properties of the Laplacian, we know that it is a quadratic form, and is hence p.s.d. Thus, it admits a decomposition $B\trans B = L$.
%
%\begin{lemma}
%Consider a $d$-regular graph $G(V,E)$. If there exists some set $|S| \le \delta|V|$ such that $\phi(S) \le \epsilon$, then there exists a vector $x$ such that $\|x\|_0 = \delta n$ with $\|Bx\|_2 \le \sqrt{\epsilon}$.
%\end{lemma}
%\begin{proof}
%Take $x$ such that $x_i = 1$ if vertex $i$ is in $S$ and $0$ otherwise. Normalize this by dividing by $\sqrt{k}$. Obviously, $\|x\|_2^2 = 1$. We are given that $\phi(S) \le \epsilon$. Using Lemma~\ref{lem:sparsecheeger}, we get $1 - \lambda_2 \le \epsilon$, which in turn gives us $\frac{x\trans G x}{d\cdot x\trans x} \ge (1 - \epsilon)$. We get $$x\trans d (I - L) x \ge (1 - \epsilon)d$$ or equivalently $$x\trans L x \le \epsilon$$
%Using the decomposition, we get $$x\trans B\trans B x = \|Bx\|_2^2 \le \epsilon$$
%\end{proof}
%
%\begin{theorem} For any $\epsilon$, there exists some $\delta $ so that it is NP-hard to distinguish the following two cases for a Diagonally Dominant PSD  matrix 
% 
%\begin{itemize}
%\item $1\geq \lambda_{\delta_1} \geq 1-\epsilon$ 
%\item $\lambda_{\delta_2} \leq \epsilon$
%\end{itemize}
%for any any $\delta_1,\delta_2 <\delta.$
%
%\end{theorem}
%\begin{proof}
%Given any SSE instance, we would let consider $I-U/d$. We know that if  
%
%\end{proof}
%\begin{theorem} Given a matrix $A$, it is NP-hard to distinguish the following two cases:
%\begin{itemize}
%\item $RIP_{k_1}(M) \leq \epsilon$.
%\item $RIP_{k_2}(M) \geq (1-\epsilon)$
%\end{itemize}
%for any $k_1,k_2\leq k(\epsilon)$
%\end{theorem}
%\begin{proof}
%We just need to consider the matrix $BB^T = (I-U/d)$.
%\end{proof}

